QBitOpt: Fast and Accurate Bitwidth Reallocation during Training

Quantizing neural networks is one of the most effective methods for achieving efficient inference on mobile and embedded devices. In particular, mixed precision quantized (MPQ) networks, whose layers can be quantized to different bitwidths, achieve better task performance for the same resource constraint compared to networks with homogeneous bitwidths. However, finding the optimal bitwidth allocation is a challenging problem as the search space grows exponentially with the number of layers in the network. In this paper, we propose QBitOpt, a novel algorithm for updating bitwidths during quantization-aware training (QAT). We formulate the bitwidth allocation problem as a constraint optimization problem. By combining fast-to-compute sensitivities with efficient solvers during QAT, QBitOpt can produce mixed-precision networks with high task performance guaranteed to satisfy strict resource constraints. This contrasts with existing mixed-precision methods that learn bitwidths using gradients and cannot provide such guarantees. We evaluate QBitOpt on ImageNet and confirm that we outperform existing fixed and mixed-precision methods under average bitwidth constraints commonly found in the literature.

==> sections/100_rebutal.tex <==
\section{Rebutal}
\input{tables/imagene_results_rebutal}

==> sections/iccv.tex <==
\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a
sentence-ending space. So \eg is correct, {\em e.g.} is not.  The provided
\verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'',
shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word.)
However, use it only when there are three or more authors.  Thus, the
following is correct: ``
   Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...''
because reference~\cite{Alpher03} has just two authors.  If you use the
\verb'\etal' macro provided, then you need not worry about double periods
when used at the end of a sentence as in Alpher \etal.

For this citation style, keep multiple citations in numerical (not
chronological) order, so prefer \cite{Alpher03,Alpher02,Authors14} to
\cite{Alpher02,Alpher03,Authors14}.

\begin{figure*}
\begin{center}
\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
\end{center}
   \caption{Example of a short caption, which should be centered.}
\label{fig:short}
\end{figure*}

%------------------------------------------------------------------------
\section{Formatting your paper}

All text must be in a two-column format. The total allowable width of the
text area is $6\frac78$ inches (17.5 cm) wide by $8\frac78$ inches (22.54
cm) high. Columns are to be $3\frac14$ inches (8.25 cm) wide, with a
$\frac{5}{16}$ inch (0.8 cm) space between them. The main title (on the
first page) should begin 1.0 inch (2.54 cm) from the top edge of the
page. The second and following pages should begin 1.0 inch (2.54 cm) from
the top edge. On all pages, the bottom margin should be 1-1/8 inches (2.86
cm) from the bottom edge of the page for $8.5 \times 11$-inch paper; for A4
paper, approximately 1-5/8 inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area 6-7/8 inches (17.5 cm) wide by 8-7/8 inches (22.54 cm)
high.

Page numbers should be included for review submissions but not for the 
final paper. Review submissions papers should have page numbers in the 
footer with numbers centered and .75 inches (1.905 cm) from the bottom 
of the page and start on the first page with the number 1.

Page numbers will be added by the publisher to all camera-ready papers 
prior to including them in the proceedings and before submitting the 
papers to IEEE Xplore. As such, your camera-ready submission should 
not include any page numbers. Page numbers should automatically be 
removed by uncommenting (if it's not already) the line
\begin{verbatim}
% \iccvfinalcopy
\end{verbatim}
near the beginning of the .tex file.

%-------------------------------------------------------------------------
\subsection{Type-style and fonts}

Wherever Times is specified, Times Roman may also be used. If neither is
available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE. Center the title 1-3/8 inches (3.49 cm) from the top edge of
the first page. The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and
adverbs; do not capitalize articles, coordinate conjunctions, or
prepositions (unless the title begins with such a word). Leave two blank
lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type. This information is to
be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT. Type main text in 10-point Times, single-spaced. Do NOT use
double-spacing. All paragraphs should be indented 1 pica (approx. 1/6
inch or 0.422 cm). Make sure your text is fully justified---that is,
flush left and flush right. Please do not place any additional blank
lines between paragraphs.

Figure and table captions should be 9-point Roman type as in
Figures~\ref{fig:onecol} and~\ref{fig:short}.  Short captions should be centered.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-,
second-, and third-order headings.

FIRST-ORDER HEADINGS. (For example, {\large \bf 1. Introduction})
should be Times 12-point boldface, initially capitalized, flush left,
with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS. (For example, { \bf 1.1. Database elements})
should be Times 11-point boldface, initially capitalized, flush left,
with one blank line before, and one after. If you require a third-order
heading (we discourage it), use 10-point Times, boldface, initially
capitalized, flush left, preceded by one blank line, followed by a period
and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote {This is what a footnote looks like.  It
often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral
observations in
the text (within parentheses, if you prefer, as in this sentence).  If you
wish to use a footnote, place it at the bottom of the column on the page on
which it is referenced. Use Times 8-point type, single-spaced.

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times,
single-spaced, at the end of your paper. When referenced in the text,
enclose the citation number in square brackets, for
example~\cite{Authors14}.  Where appropriate, include the name(s) of
editors of referenced books.

\begin{table}
\begin{center}
\begin{tabular}{|l|c|}
\hline
Method & Frobnability \\
\hline\hline
Theirs & Frumpy \\
Yours & Frobbly \\
Ours & Makes one's heart Frob\\
\hline
\end{tabular}
\end{center}
\caption{Results.   Ours is better.}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.  Please ensure that any point you wish to
make is resolvable in a printed copy of the paper.  Resize fonts in figures
to match the font in the body text, and choose line widths that render
effectively in print.  Many readers (and reviewers), even of an electronic
copy, will choose to print your paper in order to read it.  You cannot
insist that they do otherwise, and therefore must not assume that they can
zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use
\verb+\includegraphics+, and to specify the  figure width as a multiple of
the line width as in the example below
{\small\begin{verbatim}
   \usepackage[dvips]{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.eps}
\end{verbatim}
}

==> tables/ema_abl.tex <==
\begin{table}[t]
\centering
\begin{tabular}{l c c c}
\toprule
Architecture & W/A & $\alpha$ & Acc. (\%) \\
\midrule
% \multirow{6}{c}{\mnv{2}} & \multirow{6}{c}{4} & 0.05 & 69.72 \\
\multirow[c]{6}{*}{\rotatebox[origin=c]{0}{\mnv{2}}} &
\multirow[c]{6}{*}{4\textsubscript{MP}} 
  & 0.05 & 69.73\textsuperscript{0.01} \\
& & 0.25 & 69.72\textsuperscript{0.08} \\
& & 0.5 & 69.72\textsuperscript{0.27} \\
& & 0.75 & 69.69\textsuperscript{0.19} \\
& & 0.9 & 69.71\textsuperscript{0.10} \\
& & 1.0 & 69.72\textsuperscript{0.12} \\
\midrule
\multirow[c]{6}{*}{\rotatebox[origin=c]{0}{EfficientNet-Lite}} &
\multirow[c]{6}{*}{4\textsubscript{MP}} 
  & 0.05 & 72.33\textsuperscript{0.11} \\
& & 0.25 & 73.29\textsuperscript{0.09} \\
& & 0.5 & 73.28\textsuperscript{0.11} \\
& & 0.75 & 73.34\textsuperscript{0.05} \\
& & 0.9 & 73.28\textsuperscript{0.05} \\
& & 1.0 & 73.34\textsuperscript{0.17} \\
\midrule
\multirow[c]{6}{*}{\rotatebox[origin=c]{0}{\mnv{3}}} &
\multirow[c]{6}{*}{4\textsubscript{MP}} 
  & 0.05 & 69.72\textsuperscript{0.10} \\
& & 0.25 & 69.72\textsuperscript{0.10} \\
& & 0.5 & 69.72\textsuperscript{0.10} \\
& & 0.75 & 69.72\textsuperscript{0.10} \\
& & 0.9 & 69.72\textsuperscript{0.10} \\
& & 1.0 & 69.72\textsuperscript{0.10} \\
\midrule
\multirow[c]{6}{*}{\rotatebox[origin=c]{0}{\mnv{3}}} &
\multirow[c]{6}{*}{3\textsubscript{MP}} 
  & 0.05 & 69.72\textsuperscript{0.10} \\
& & 0.25 & 69.72\textsuperscript{0.10} \\
& & 0.5 & 69.72\textsuperscript{0.10} \\
& & 0.75 & 69.72\textsuperscript{0.10} \\
& & 0.9 & 69.72\textsuperscript{0.10} \\
& & 1.0 & 69.72\textsuperscript{0.10} \\
\bottomrule
\end{tabular}
\caption{\mnv{2} on ImaneNet. DQ~\cite{Uhlich2020DiffQ} results for different regularization strength $\lambda$, including our QBitOpt }
\label{tbl:ema_alpha}
\end{table}

==> tables/imagenet_results.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{ c | l | c | c | c }
    \toprule
 &   Method & W/A &  Avg. Bits & Acc. (\%)    \\
\midrule
% \multirow[c]{6}{*}{\mnv{2}}  
\multirow[c]{8}{*}{\rotatebox[origin=c]{90}{\mnv{2}}}  
 & Full-precision & 32/32 & - & 71.72  \\
\cmidrule{2-5}
 & LSQ \cite{Esser2020LSQ}      & 4/4 & - & 69.45  \\
 & DQ \cite{Uhlich2020DiffQ}    & \mpb{4/4} & 4.07 & 68.50  \\
 & QBitOpt (ours)               &  \mpb{4/4} & \textbf{4.0} & \textbf{69.71}   \\
\cmidrule{2-5}
 & LSQ \cite{Esser2020LSQ}      & 3/3 & - & 65.17   \\
  & DQ \cite{Uhlich2020DiffQ}   & \mpb{3/3} & 3.11 & 64.94  \\
 & QBitOpt (ours)               &  \mpb{3/3} & \textbf{3.0} & \textbf{65.65}  \\
%
\midrule \midrule
% \multirow[c]{6}{*}{\mnv{3}-Small} 
\multirow[c]{8}{*}{\rotatebox[origin=c]{90}{\mnv{3}-Small} }
& Full-precision & 32/32 & - & 67.67  \\
\cmidrule{2-5}
& LSQ \cite{Esser2020LSQ}       & 4/4 & - & 61.58 \\
& DQ \cite{Uhlich2020DiffQ}     & \mpb{4/4} & 4.09 & 63.61  \\
 & QBitOpt (ours)               & \mpb{4/4}   & \textbf{4.0} & \textbf{64.23}  \\
\cmidrule{2-5}
  & LSQ \cite{Esser2020LSQ}     & 3/3 & - & 51.92 \\
& DQ \cite{Uhlich2020DiffQ}     & \mpb{3/3} & 3.21 & \textbf{58.32}  \\
& QBitOpt (ours)                & \mpb{3/3}  & \textbf{3.0} & 57.14  \\
%
\midrule \midrule
\multirow[c]{8}{*}{\rotatebox[origin=c]{90}{\efnet{lite}}}
& Full-precision & 32/32 & - & 75.42  \\
\cmidrule{2-5}
 & LSQ \cite{Esser2020LSQ}      & 4/4 & - & 72.93  \\
  & DQ \cite{Uhlich2020DiffQ}   & \mpb{4/4} & 4.08 & 68.50  \\
  & QBitOpt (ours)              & \mpb{4/4} & \textbf{4.0} & \textbf{73.43}  \\
\cmidrule{2-5}
 & LSQ \cite{Esser2020LSQ}      & 3/3 & - & 69.62  \\
 & DQ \cite{Uhlich2020DiffQ}    & \mpb{3/3} & 3.12 & 68.86  \\
 & QBitOpt (ours)               & \mpb{3/3} & \textbf{3.0} & \textbf{70.04}  \\
\bottomrule
\end{tabular}
\vspace{0.2em}
 \caption{Comparison of QBitOpt with other methods on the ImageNet image classification benchmark. We report validation accuracy (\%), target \bwt (W/A) set for the corresponding method and actually achieved average \bwt (Avg. Bits) in the case of mixed precision.
 }
 \label{tbl:imagenet_results}
\end{table}

